Multi-Fidelity Multi-Armed Bandits Revisited

We study the multi-fidelity multi-armed bandit (MF-MAB), an extension of the canonical multi-armed bandit (MAB) problem. MF-MAB allows each arm to be pulled with different costs (fidelities) and observation accuracy. We study both the best arm identification with fixed confidence (BAI) and the regret minimization objectives. For BAI, we present (a) a cost complexity lower bound, (b) an algorithmic framework with two alternative fidelity selection procedures, and (c) both procedures' cost complexity upper bounds. From both cost complexity bounds of MF-MAB, one can recover the standard sample complexity bounds of the classic (single-fidelity) MAB. For regret minimization of MF-MAB, we propose a new regret definition, prove its problem-independent regret lower bound $\Omega(K^{1/3}\Lambda^{2/3})$ and problem-dependent lower bound $\Omega(K\log \Lambda)$, where $K$ is the number of arms and $\Lambda$ is the decision budget in terms of cost, and devise an elimination-based algorithm whose worst-cost regret upper bound matches its corresponding lower bound up to some logarithmic terms and, whose problem-dependent bound matches its corresponding lower bound in terms of $\Lambda$.

==> sections/_ICML_rebuttal.tex <==
% !TeX root = ..\mf-mab.tex
\section{Rebuttal for ICML Reviewers}

\subsection{Reply to Reviewer 1NQo}

\begin{enumerate}
    \item \reviewquote{Assuming the error upper bounds are known may not be true in the practical problems. If these error bounds are not tight enough, it won't be helpful as it can make a sub-optimal arm better than the optimal arm (e.g., it can violate Assumption 3.3, which is already very restrictive).}

          \answer{\textbf{Factual error.} We note that even when the error bounds are loose, the sub-optimal arm cannot be better than the optimal arm, because at the highest fidelity one can estimate the true reward means whose error bounds are zero. Therefore, Assumption 3.3 can hold and there is no contradiction between our assumptions.}

    \item \reviewquote{
              There are better algorithms than LUCB (e.g., KL-LUCB, Track-and-Stop) for best arm identification. It is unclear why the authors used the LUCB algorithm.}

          \answer{We note that the KL-LUCB is similar to LUCB except that KL-LUCB uses the KL-UCB index (a finer upper bound than UCB used in LUCB). Given our LUCB algorithm design and analysis, one can straightforwardly extend it to KL-LUCB. Because the Track-and-Stop algorithm is based on a tight sample complexity lower bound, it is non-trivial to generalize it to our multi-fidelity case whose sample cost lower bound may not be tight.}


    \item \reviewquote{
              Two (A and B) of three fidelity selection procedures may not be practical. Procedure A needs to know the threshold upfront (there is no optimal problem-dependent method to set these thresholds discussed in the paper). Whereas Procedure B assumes the true mean of the optimal arm's reward and the best suboptimal arm's reward is known, which may not be practical (as the authors also mentioned in the paper).}

          \answer{
              NAN
          }

    \item \reviewquote{
              Assuming the high-cost arm's option has higher accuracy than all low-cost options may not always be true, as a linear model may perform better than a simple neural network (in hyperparameter optimization).}

          \answer{ \qw{We kindly remind the reviewer that ``the high-cost arm's option has higher accuracy than all low-cost options" is actually not a very precise characterization of our assumption. Although quite subtle, it is important to distinguish the concept of an arm pulled at different fidelities vs. arms with different costs.  Our accuracy error bound assumption is imposed on each particular arm with different ``fidelities" (not just arms with different costs, although obtaining observations with higher fidelity typically implies a higher cost). The example the reviewer mentioned with a linear model and simple neural network is more suitable as an example case where different arms have different costs and different accuracy. But the `fidelity' concept is missing. Perhaps a more relevant example that has the fidelity concept is a neural network trained with a large number of epochs (yielding higher fidelity observation) vs. a smaller number of epochs (yielding lower fidelity observation). } Although there may be some special cases where the high fidelities cannot yield observations with higher accuracy, far more cases in hyperparameter optimization fulfill our assumption, for example, most results in the neural architecture search benchmarks \texttt{HPOBench}~\cite{eggensperger2021hpobench}, and \texttt{YAHPO Gym}~\cite{pfisterer2022yahpo} fulfills the assumption that paying high cost generates observations with higher accuracy.}


    \item \reviewquote{
              Regret minimization algorithm based on arm elimination (if there are more than two arms, pull the highest fidelity option; otherwise, pull the lowest fidelity option) is very trivial as there is no way to exploit low-fidelity options, which can keep arm pulling cost low. Further, no experimental results to show how the proposed algorithm will perform compared to the existing algorithm (Kandasamy et al., 2016b).
          }

          \answer{
              We note that there are real-world applications, e.g., the advertisement distribution problem in Section 4.3, where the explorations are conducted at the high fidelity (e.g., a large-scale user study) and the exploitations are conducted at the low fidelity (e.g., advertisement distribution via some platforms). This corroborates our algorithm design.
              On the other hand, since our algorithm enjoys the tight regret performance comparing to regret lower bound with respect to decision budget \(\Lambda\), its exploration-exploitation mechanism also implies that the approach used in real-world advertisement distribution is reasonable.}


    \item \reviewquote{
              The proposed problem has many practical applications, but most of these applications may have an infinite number of arms, e.g., hyperparameter configurations. Therefore, assuming finite arms make proposed algorithms less practical.}

          \answer{Although there are applications with infinite number of arms, many other applications have a finite number of arms, especially in the context of neural architecture search, where arms are different combinations of architecture designs. For example, the hyperparameter configurations reported in the neural architecture search benchmarks \texttt{HPOBench}~\cite{eggensperger2021hpobench} and \texttt{YAHPO Gym}~\cite{pfisterer2022yahpo} is a finite number of choices. In addition, for applications with an infinite number of arms, it is also common to discretize the arm space and transform it to a finite number of arms.}

    \item \reviewquote{
              Describing suitable motivational examples (matches with the problem setting) in the introduction (instead of doing it later) will help to motivate the reader about the problem.
          }

          \answer{We thank the reviewer for this instructive suggestion. We will move forward two motivation examples (one for BAI, one for regret) to introduction in the final version of this paper.}

\end{enumerate}


\subsection{Reply to Reviewer x9Ni}


\begin{enumerate}
    \item \reviewquote{
              Is the second term in the upper bound in (9) unavoidable?
              For best arm identification, there is no lower bound that matches the second term in (9). Moreover, the lower bound is in terms of the minimum ratio while the upper bound is in terms of the ratio at m given after equation (9).
          }

          \answer{Yes, the second term of Eq.(9) is unavoidable in the current algorithm design. Recently, we devised a modified algorithm in whose sample cost upper bound we can remove the second term. We will add this new result into a journey version of this paper. For the mismatch in term of the fidelity in Eq.(9) comparing to the lower bound, we note that the optimal fidelity used in Eq.(10) (for \textsc{FidelitySelection}-B) is the same as the fidelity in our lower bound. }

    \item \reviewquote{Is the dependency on K in Theroem 4.3 optimal?
              For regret minimization, the lower bound does not consider the dependency on the number of arms K which is often an interesting part of the lower bound proof.}

          \answer{We highly appreciate this suggestion. We will leave the dependency on the number of arms \(K\) of lower bound as a further direction in the conclusion in the final conference version of this paper and look into it in a future journal version of this paper.}

    \item \reviewquote{What is \(\nu\) in Theorem 3.1?     Some parts of the paper are poorly written. For example, what is the
              in the statement of the lower bound (Theorem 3.1)? I could not find its definition.}

          \answer{Thanks for pointing out this missing defintion. The \(\nu\) denotes the reward distribution assocated to arms. For example, the \(\nu_k\upbra{m}\) represents the the reward distribution of arm \(k\) when pulled at fidelity \(m\).
              We will add this definition and also double-check the whole paper's notation definitions in the final version of this paper.}
\end{enumerate}


\subsection{Reply to Reviewer uk23}


\begin{enumerate}
    \item On Theorems 3.1 and 3.4: \begin{itemize}
              \item \reviewquote{
                        In Algorithm 2A, how is \(\gamma\) chosen? It seems like this is critical to the performance of the algorithm and the bounds? Is there an optimal way to pick these parameters?}

                    \answer{
                        We would suggest to set \(\gamma\upbra{m}\) as \(\zeta\upbra{m}\) because the \(\gamma\upbra{m}\) is a lower bound of the confidence radius of reward mean estimate at fidelity \(m\) in \textsc{FidelitySelection}-A,
                        and allowing the confidence radius to be smaller than the error bound \(\zeta\upbra{m}\) can hardly help to improve the algorithm's performance.
                        We agree that the selection of \(\gamma\upbra{m}\) is crucial for the performance of Algorithm 2 with \textsc{FidelitySelection}-A, and we do not figure out whether there exists an optimal way to pick them.
                    }

              \item \reviewquote{
                        What is the interpretation of the quantity \(G^*\) in Theorem 3.4 (B)? It is looking at the inverse squared difference of the normalized gaps? This quantity maybe quite large, at least as large as the sum of the inverse squared normalized gaps? How do you conclude that even this oracular algorithm is optimal for this setting?}

                    \answer{The \(G^*\log(\log 1/\delta)\) term in Theorem~\ref{thm:proc-b} stands for the cost of finding the optimal fidelities \(m_k^*\) of all arms. Because finding the optimal fidelity \(m_k^* = \argmax_{m\in\mathcal{M}} {\Delta_k\upbra{m}}/{\sqrt{\lambda\upbra{m}}}\) requires one to comparing \({\Delta_k\upbra{m}}/{\sqrt{\lambda\upbra{m}}}\) of different fidelities, the \(G^*\) contains \textit{``the inverse squared difference of the normalized gaps.''}
                    We agree that this quantity \(G^*\) can be very large,
                    and we did not claim that our sample cost upper bound is optimal.
                    We will add a discussion about the quantity \(G^*\) as above in the final version of this conference paper.\\
                    It is worth noting that we recently devise a modified algorithm in whose sample cost upper bound we remove the second term containing \(G^*\). We will add this new result into a journey version of this paper.
                    }


              \item \reviewquote{
                        The lower bound result for the BAIc setting appears straightforward from existing results. However, it apears that it is also loose. This can be inferred from the fact that it doesn't capture the cost for discovering the best fidelity at which to explore an arm, and that only an algorithm which has oracular knowledge of the arm means can achieve this lower bound (more on this below). The authors also seem to acknowledge this.
                    }

                    \answer{NAN}
          \end{itemize}


    \item  On Theorems 4.2 and 4.3: \reviewquote{
              The theorems present a \(\Lambda^{2/3}\) worst case lower and upper bound for the cumulative regret. The issue is that it is easy to design an algorithm that achieves a \(\Lambda^{2/3}\) regret: use an explore-then-commit strategy which explores at the most expensive fidelity and then exploits at the cheapest fidelity. Hence, I am not sure if a worst-case result is interesting here. It might be more instructive to see some bounds that have a more nuanced dependence on the problem parameters (e.g costs, \(\zeta\)'s, and gaps). The authors' algorithm is probably doing something smarter that n this, but it should be made clear via the regret bounds.}


          \answer{
              We derived problem-dependent regret bounds.
              For Algorithm~\ref{alg:elimination-for-rm}, we derived its problem-dependent regret upper bound in Eq.\eqref{eq:prob-dep-regret-upper-bound} at Appendix~\ref{subapp:regret-upper-bound}. If we let a parameter \(\epsilon\) in the bound goes to zeros and set the decision budget \(\Lambda\) to be infinity, the upper bound becomes \[
                  \limsup_{\Lambda\to\infty }\frac{\E\left[ R(\Lambda) \right]}{\log (\Lambda)} \le  \sum_{k\in \mathcal{K}}
                  \left( \frac{\lambda\upbra{M}}{\lambda\upbra{1}} \mu_1\upbra{M} - \mu_k\upbra{M} \right)
                  \frac{16}{(\Delta_k\upbra{M})^2}.
              \]
              We also derived a problem-dependent regret lower bound for our new regret definition as follows, \[
                  \liminf_{\Lambda\to\infty }\frac{\E\left[ R(\Lambda) \right]}{\log (\Lambda)} \ge  \sum_{k\in \mathcal{K}} \min_{m:\Delta_k^{(m)}>0} \left( \frac{\lambda\upbra{m}}{\lambda\upbra{1}} \mu_1\upbra{M} - \mu_k\upbra{M} \right)\frac{C}{(\Delta_k^{(m)})^2}.
              \]
              The key different between the lower and upper bounds is that
              in the upper bound, all arms are explored at the highest fidelity \(M\),
              while the lower bound suggests that for exploring an arm there exists an optimal high fidelity which is not necessary to be the highest one.\\
              The problem-dependent lower bound was not presented in the current version of this paper, because we thought the \(\Lambda^{2/3}\) result was more interesting comparing to the \(T^{1/2}\) worst-cost bound in traditional bandits.
              We will add both problem-dependence bounds and their comparison to the main text in the final version of this paper.}

    \item Other comments: \reviewquote{
              You should probably explain what the \(\mathcal{M}_k\) terms in Theorem 3.1 in words and more clearly. It took me a long time to understand what those quantities meant.}

          \answer{Thank you for your suggestion. We will add a sentence to explain the definition of \(\mathcal{M}\) as follows, \\
              ``... the \(\mathcal{M}_k\) is a subset of fidelities \(\mathcal{M}\) containing the highest fidelity \(M\), i.e.,
              \(\mathcal{M}_k\in 2^\mathcal{M}\) and \(M\in \mathcal{M}_k\), for all \(k\in\mathcal{K}\) ...''}
\end{enumerate}

==> sections/_regret_min_half.tex <==
% !TeX root = ..\mf-mab.tex
\section{A Necessary and Sufficient Assumption for Achieving \(\Theta(\Lambda^{\frac{1}{2}})\) Regret Bound}\label{subsec:half-regret-bound}

\begin{assumption}\label{asp:half-lambda-lower-bound-condition}
    The multi-fidelity bandits with regret objective in~\eqref{eq:lambda1-regret}
    has the \(\Omega(\Lambda^\frac{1}{2})\)
    regret lower bound if the following conditions hold together: \begin{enumerate}
        \item There exists an \(\ell \in \mathcal{K}\) and a constant \(C>0\) such that for any instance \(I\), we have
              (a) \(k^{(1)}_{\ell^{\text{th}}} (I) = k^{(M)}_\bigstar (I)\), where \(k^{(1)}_{\ell^{\text{th}}}\) is the \(\ell^{\text{th}}\) best arm in the fidelity \(1\)
              and \(k^{(M)}_\bigstar\) is the optimal arm in the fidelity \(M\),
              and (b) \(\frac{\Delta^{(M)}_k(I)}{\tilde{\Delta}^{(1)}_{k,\ell^{\text{th}}}(I)} \le C\) for any arm \(k\) with \(\tilde{\Delta}^{(1)}_{k,\ell^{\text{th}}}(I) > 0\),
              where the \(\tilde{\Delta}^{(1)}_{k,\ell^{\text{th}}} \coloneqq
              \abs{\mu_{\ell^\text{th}}^{(1)} - \mu_k^{(1)}}\)
              and \(\mu^{(1)}_{\ell^{\text{th}}}\) is the \(\ell^{\text{th}}\) best arm's reward mean in fidelity \(1\);
              and
        \item The \(\ell\) in the previous condition is known a priori.
    \end{enumerate}
\end{assumption}

Theorem~\ref{thm:half-bound-necessary-condition} illustrates that Assumption~\ref{asp:half-lambda-lower-bound-condition} is necessary.

\begin{theorem}\label{thm:half-bound-necessary-condition}
    If any of Assumption~\ref{asp:half-lambda-lower-bound-condition}'s conditions fails, the worst case regret is lower bounded by \(\Omega(\Lambda^\frac{2}{3})\), that is, the \(\Omega(\Lambda^\frac{1}{2})\) bound is unreachable.
\end{theorem}

Next, we devise Algorithm~\ref{alg:half-bound-sufficient-condition}---which utilizes Assumption~\ref{asp:half-lambda-lower-bound-condition}
and achieves the \(O(\Lambda^\frac{1}{2})\) regret upper bound (Theorem~\ref{thm:half-bound-sufficient-condition})---to illustrate that Assumption~\ref{asp:half-lambda-lower-bound-condition} is also sufficient for the \(O(\Lambda^\frac{1}{2})\) bound.

Algorithm~\ref{alg:half-bound-sufficient-condition} utilizes the successive accept and reject approach~\cite{bubeck2013multiple} originally designed for best arm identification
to find the \(\ell^\text{th}\) best arm. After finding the \(\ell^\text{th}\) best arm in fidelity \(1\), the algorithm keeps pulling this arm and thus achieves the regret minimization objective.
We present its regret upper bound in Theorem~\ref{thm:half-bound-sufficient-condition}.

\begin{algorithm}[H]
    \caption{A Variant of Successive Accept and Reject}
    \label{alg:half-bound-sufficient-condition}
    \begin{algorithmic}[1]
        \STATE \textbf{Initialization: }
        Candidate arm set \(\mathcal{D} \gets \mathcal{K}\),
        accepted arms' counter \(L\gets \ell\).
        \WHILE{\(t\le T\)}
        \STATE Pull each arm in \(\mathcal{D}\) once
        \STATE \(I_t\gets\) the \(L^{\text{th}}\) empirical optimal arm
        \IF{\(\LCB(I_t) > \UCB(k)\) for some arm \(k\in\mathcal{D}\)}
        \STATE \(\mathcal{D}\gets\mathcal{D}\setminus\{k\}\) \COMMENT{reject arm \(k\)}
        \ENDIF
        \IF{\(\UCB(I_t) < \LCB(k)\) for some arm \(k\in\mathcal{D}\)}
        \STATE \(L\gets L-1\)
        \STATE \(\mathcal{D}\gets\mathcal{D}\setminus\{k\}\) \COMMENT{accept arm \(k\)}
        \ENDIF
        \ENDWHILE
    \end{algorithmic}
\end{algorithm}

\begin{theorem}\label{thm:half-bound-sufficient-condition}
    Under Assumption~\ref{asp:half-lambda-lower-bound-condition}, the regret of Algorithm~\ref{alg:half-bound-sufficient-condition} is upper bounded as follows, \[
        \E\left[ R(\Lambda) \right] \le O(\Lambda^\frac{1}{2}).
    \]
\end{theorem}
